Expressive Power of Broadcast Consensus Protocols

Population protocols are a formal model of computation by identical, anonymous mobile agents interacting in pairs. Their computational power is rather limited: Angluin et al. have shown that they can only compute the predicates over $\mathbb{N}^k$ expressible in Presburger arithmetic. For this reason, several extensions of the model have been proposed, including the addition of devices called cover-time services, absence detectors, and clocks. All these extensions increase the expressive power to the class of predicates over $\mathbb{N}^k$ lying in the complexity class NL when the input is given in unary. However, these devices are difficult to implement, since they require that an agent atomically receives messages from all other agents in a population of unknown size; moreover, the agent must know that they have all been received. Inspired by the work of the verification community on Emerson and Namjoshi's broadcast protocols, we show that NL-power is also achieved by extending population protocols with reliable broadcasts, a simpler, standard communication primitive.

==> sec-anonymity-indistinguishability.tex <==
\newcommand{\Id}{\textit{Id}}

We compare the models mentioned in this paper: community protocols,
mediated protocols, broadcast protocols (as a representative of the class of oblivious protocols, as expressive as any other), and population protocols. While the comparison is
technically simple, it requires to define some notions with precision.

All four models postulate a finite set of states $Q$, input alphabet
$\Sigma$, and input and output functions $I, O$. However, not all
assume that agents have no identities, or that only agents can store
information.

\parag{Community protocols} assume an infinite set $\Id$ of \emph{agent
  iden\-tifiers}, e.g. $\N$, and a total order
$\prec\ \subseteq \Id \times \Id$, e.g., the natural order $<$.
Each agent is assigned a unique identifier, and so for $a \in \Id$, we
speak of ``the agent $a$''.
Each agent can store up to a constant
number of identifiers. At each step, two agents, say $a_1, a_2$,
interact and move to new states. Assume $a_1$ and $a_2$ are in states
$q_1, q_2$ with store values $A_1, A_2$. The new states $q_1', q_2'$
and store values $A_1', A_2'$ are a function of $q_1, q_2,
a_1, a_2, A_1, A_2$. However, the function only depends on $\prec
\cap~(A \times A)$, where $A = \{a_1, a_2\} \cup A_1 \cup A_2$, and not on the set $A$ itself
(technically, the function must return the same value for any two sets $A, A'$ such that there is a
$\prec$-preserving bijection between $A$ and $A'$).
 A possible transition of a community protocol is:
\begin{quote}
  If agents $a_1$ and $a_2$ are in state $p$, and $a_1 \prec a_2$,
  then agents $a_1$ and $a_2$ can move resp.\ to states $q_1$ and $q_2$.
\end{quote}

\parag{Mediated protocols} postulate a set of agents communicating by
means of point-to-point channels, one for each pair of
agents. Channels have a constant amount of memory. This is formalized
by introducing a set $Q$ of agent states and a disjoint set $S$ of
channel or \emph{edge} states. Transitions are of the form $(q_1, q_2,
s) \mapsto (q_1', q_2', s')$, with the following meaning:

\begin{quote}
  If two agents are in state $q_1$ and $q_2$, and the channel between
  them is in state $s$, then the agents move to states $q_1'$ and
  $q_2'$, and the channel moves to state $s'$.
\end{quote}

Observe that the transitions, and hence the step relation induced by
them, do not depend on the identifiers of the agents.

A first axis for the comparison are the privacy properties preserved
by the different classes. In particular, one of the motivations for
mediated protocols was to design a model with expressive power similar
to the power of community protocols, but satisfying anonymity, which
was however not formally defined in~\cite{MCS11}. While for the purposes
of~\cite{MCS11} this is no problem, we need a definition here to
compare anonymity with a second natural property, \emph{indistinguishability}, which holds for
oblivious protocols, but not for mediated or community
protocols\footnote{We remark that privacy issues in population protocols have
also been studied in~\cite{DelporteGalletFGR07}, albeit in a
different context, in which agents should not be able to learn the
input values of other agents.}.

The second axis of the comparison is the expressive power of the
models. Together with the first axis, it describes the price of
privacy. We determine for each model the class of predicates
computable by the model. For the comparison, we need a uniform
definition of ``a protocol computes a predicate''. Fortunately,
Definition~\ref{def:comp-pred} applies to all models. In particular,
recall that a predicate $\varphi$ of arity 1 is
computable by a class of protocols if there is a protocol in the class
such that for every number $n$, the value $\varphi(n)$ can be computed
by the protocol with $n$ agents in the unique initial
state.

\subsection{Defining anonymity and indistinguishability}
Let $\Id$ be a set of identifiers or names, and let $Q$ be a set of
states. A \emph{trajectory} is a finite sequence of states. A
\emph{trace} of length $k$ is a mapping $\tau$ that assigns to every
$a \in \Id$ a trajectory $\tau(a)$ of length $k$. A \emph{trace
  language} is a set of traces (possibly of different lengths). In the
rest of the section, we identify a protocol with the set of traces it
can execute, defined in the expected way.

Intuitively, anonymity guarantees that by observing the trajectories
of the agents in one execution, one cannot gain any information about
their identities.

Given a trace $\tau$ and a permutation $\pi \colon \Id \to \Id$, we
define $\tau \circ \pi$ as the trace given by $(\tau \circ \pi)(a)
\defeq \tau(\pi(a))$.

\begin{definition}
  A trace language $L$ \emph{preserves anonymity} if $\tau \in L \iff
  (\tau \circ \pi) \in L$ for every trace $\tau$ and permutation
  $\pi$.
\end{definition}

Now we introduce a second property, called indistinguishability. To
motivate it, consider a ``House of Cards'' protocol with the following
states:

\begin{center}
  \begin{tabular}{l|l}
    State & Intended meaning \\ \hline
    $M$   & ``agent knows that the US president is a Murderer'' \\
    $N$   & ``agent knows Nothing'' \\
    $C$   & ``agent goes to the Cinema'' \\
    $J$    & ``agent talks to a Journalist'' \\
    $D$   & ``agent Dies of a heart attack''
  \end{tabular}
\end{center}

\noindent Assume a detective informs the president that two agents
have executed the trajectories $\{M C J, N C D\}$. Even if the
president ignores the identities of the agents, s/he has learned
crucial information. Imagine now the agents are identical twins. The
detective observes that both enter the cinema and later, at the end of
the film, leave it. In this case, the detective and president only
learn that the trajectories are either $\{M C J, N C D\}$ or $\{M C D,
N C J\}$, a very different situation!
In the twin case, agents that occupy the same state at the same time
are indistinguishable: We may know the set of their past and future
trajectories, but not how these two sets are connected. We call this
property \emph{indistinguishability}. Let us formalize it. Given two
traces $\tau_1$ and $\tau_2$, define their concatenation $\tau_1
\tau_2$ by $(\tau_1 \tau_2)(a) \defeq \tau_1(a) \tau_2(a)$ for every
$a \in \Id$. A permutation is \emph{compatible} with $\tau$ if for
every $a \in \Id$, the trajectories $\tau(a)$ and $\tau(\pi(a))$ start
in the same state.

\begin{definition}
  A trace language $L$ \emph{preserves indistinguishability} if for
  every two traces $\tau, \tau'$ and for every permutation $\pi$
  compatible with $\tau'$, we have: $\tau\tau' \in L \iff \tau (\tau'
  \circ \pi) \in L$.
\end{definition}

It follows immediately from the definition that oblivious consensus
protocols preserve indistinguishability. The converse does not hold:
Indeed, one can design protocols in which the step relation depends
not only on the current configuration, but also on previous
ones. Those protocols preserve indistinguishability, but are not
oblivious. In fact, the following ``equation'' is a direct consequence of the
definitions:
\begin{center}
  Obliviousness = Indistinguishability + Memorylessness,
\end{center}
\noindent where memorylessness means that steps from a configuration
$C$ depend only on $C$, and not on the past of the
computation.

\subsection{Comparison}

We go through the four models, describing the privacy properties they
satisfy and their computational power.

\subsubsection{Community protocols}

Community protocols do not preserve anonymity.

\begin{example}
  Consider a community protocol with $\{p, q_1, q_2\}$ as set of
  states and the following unique transition:
  \begin{quote}
    If agents $a_1$ and $a_2$ are in state $p$, and $a_1 \prec a_2$,
    then agents $a_1$ and $a_2$ can move resp.\ to states $q_1$ and $q_2$.
  \end{quote}
  Mapping $\tau$ with $\tau(a_1)= p \, q_1$ and $\tau(a_2) = p \, q_2$
  is a trace of the protocol, but $\tau \circ \pi$ with $\pi(a_1)=a_2,
  \pi(a_2)=a_1$ is not.
\end{example}

In~\cite{GR09}, Guerraoui and Ruppert show the following result. Let
$M$ be a nondeterministic Turing machine, over alphabet $\Sigma$,
running in $O(n \log n)$ space. There is a community protocol such
that, for every input word $w \in \Sigma^*$ of length $n$, the
following holds: $M$ accepts $w$ (resp.\ rejects $w$) if{}f
the instance of the protocol in which $n$ agents with identities $1,
2, \ldots, n$ are initially put in states $I(w_1), I(w_2), \ldots,
I(w_n)$ converges to $1$ (resp.\ to $0$). Moreover, the $O(n \log n)$
space bound is tight, i.e., the property does not hold for any
function $f \in \omega(n \log n)$.

Guerraoui and Ruppert state their result as ``community protocols
compute exactly the predicates in $O(n \log n)$''. However, in our
setting the result is actually far more impressive. Indeed, consider
any predicate $\varphi \in \NSPACE(2^{n \log n})$ of arity
$k$. For such a predicate, there is a Turing machine $M$ running in
$\bigO(n \log n)$-space such that for every $\vec{x} \in \N^k$, the
machine accepts the unary encoding of $\vec{x}$, i.e.\ $w =
1^{\vec{x}_1} \# 1^{\vec{x}_2} \# \cdots \# 1 ^{\vec{x}_k}$, if{}f
$\varphi(\vec{x}) = 1$. By the result of~\cite{GR09}, the execution of
$M$ on $w$ can be simulated by the instance of a community protocol
with a total of $\vec{x}_1 + \vec{x}_2 + \ldots + \vec{x}_k$ agents;
more precisely, for every $1 \leq i \leq k$ we place $\vec{x}_i$
agents in the state corresponding to the $i$-th input. Therefore, we
obtain:

\begin{proposition}[\cite{GR09}]
  Community protocols compute exactly the predicates contained
  in $\NSPACE(2^{n \log n})$.
\end{proposition}

\subsubsection{Mediated protocols}

Since, by definition, transitions of mediated protocols do not depend
on agent identities, mediated protocols satisfy anonymity. However,
they do not satisfy indistinguishability. It is easy to construct an
instance of a mediated protocol with three agents, two twins $a,
b$ and a detective $d$, modeling the ``House of Cards''
scenario. In addition to the states $M,N,C,J,D$ of the twins,
the detective can be in states $F$ (follow) and $K$ (Kill). The detective is
initially in state $F$ (follow), the twins
in states $M$ and $N$. All transitions involve a twin and the
detective. When the twins go to the cinema, the detective updates the
state of their communication channel by means of transitions $(M, F,
0) \mapsto (C, F, 1)$ and $(N, F, 0) \mapsto (C, F, 0)$,
respectively. This amounts to ``tagging'' the twin in state $M$ with a
$1$ before she enters the cinema, and tagging her sister with a $0$.
Transition $(C, F, 1) \mapsto (J, K, 1)$ allows the detective to know
that the dangerous twin is the one that after exiting the cinema is meeting the journalist, and hence
to move to state Kill.  The appendix describes the mediated protocol in detail, and
describes a trace $\tau \, \tau'$ of the protocol such that $\tau (\tau' \circ \pi)$ is not a trace,
where $\pi$ is a the mapping that permutes the twins. Intuitively, $\tau$ and $\tau'$ describe
the behavior before and after entering the cinema.

In \cite{MCS11}, Michail, Chatzigiannakis and Spirakis show that a
mediated protocol can simulate a Turing machine running in
$\NSPACE(n^2)$. Applying the same observations as for community
protocols, we obtain:

\begin{proposition}[\cite{MCS11}]
  Community protocols compute exactly the predicates contained
  in $\NSPACE(2^{n^2})$.
\end{proposition}

This shows that anonymity can be achieved without losing expressive
power. (The fact that the expressive power looks even higher is due to
the fact that channels are not considered as agents, even though they
have states.)

\subsubsection{Broadcast protocols}

Oblivious protocols preserve anonymity and indistinguishability. This
follows immediately from the definition. As we have seen,
(reasonable) oblivious protocols can only compute predicates in
$\NSPACE(n)$. Broadcast protocols reach the theoretical bound, while
population protocols stay ``exponentially far'' from it, and can only
compute predicates in $\DSPACE(\log n)$.

It was shown in~\cite{BlondinEJ18} that extending the population
protocol model with interactions between $k$ agents, for any fixed
$k$, does not increase the expressive power. So the main difference
between population and broadcast protocols is the fact that the latter
exhibit \emph{global} interactions involving \emph{all} agents.

%% It was shown in~\cite{BlondinEJ18} that extending the population
%% protocol model with $k$-way interactions for any fixed $k$ (i.e.,
%% interactions between $k$ agents) does not increase the expressive
%% power. So the main difference between population and broadcast
%% protocols is the fact that the latter exhibit \emph{global}
%% interactions involving \emph{all} agents.

\subsubsection{Population protocols}
Population protocols preserve anonymity and indistinguishability, because they are
oblivious. Their interactions, however, involve ony a constant number of agents.
We prove that their expressive power is expoenntially lower than that of broadcast
protocols.


\begin{proposition}\label{prop:PA}
  For every Presburger formula $\varphi$, it is the case that $\varphi
  \in \DSPACE(\log n)$.
\end{proposition}

\begin{proof}
  Let us fix some Presburger formula $\varphi$ with $d$ free
  variables. We must show that there exists a deterministic logspace
  Turing machine that accepts $L_\varphi$. We first describe a
  language closely related to $L_\varphi$. Let $\Sigma \defeq \{0,
  1\}^d$, let $\vec{x}_\varepsilon \defeq \vec{0}$ and, for every word
  $w \in \Sigma^+$, let $\vec{x}_w \in \N^d$ be such that
  $$\vec{x}_w(i) \defeq \val(w_1(i) \cdot w_2(i) \cdots w_{|w|}(i))$$
  where $\val(u)$ is the numerical value of $u$ interepreted as a
  binary sequence with its most significant bit first. For example,
  the vector $\vec{x}_w$ associated to $w = (1,0)(1,1)(0,0)(1,1)$ is
  $(13, 5)$ since ${1101}_2 = 13$ and ${0101}_2 = 5$.

  Since $\varphi$ is a Presburger formula, there exists a
  deterministic finite automaton $A$ that accepts the language
  $$
  X_\varphi \defeq \{w \in \Sigma^* : \varphi(\vec{x}_w) = 1\}.
  $$
  Note that the usual constructions to translate a Presburger formula
  into an automaton yield a \emph{nondeterministic} finite automaton
  $B$ with \emph{least-significant}-bit-first encoding (see
  e.g.~\cite{BoudetC96}). This is not an issue since the language of
  $B$ can be reversed and the resulting automaton can be determinized,
  by standard results on regular languages.

  Observe that a Turing machine can decide whether $\varphi(\vec{x}) =
  1$ by simulating $A$ on the binary encoding of $\vec{x}$. However,
  we have to be careful since the encoding of $\vec{x}$ in $X_\varphi$
  and $L_\varphi$ differ: $X_\varphi$ interleaves the bits of each
  component of $\vec{x}$, while $L_\varphi$ does not. With this in
  mind, let us give a deterministic Turing machine $M$ for
  $L_\varphi$:

  \begin{enumerate}
  \item $M$ receives an input $\bin(n_1) \# \bin(n_2) \# \cdots \#
    \bin(n_d)$;

  \item $M$ has a counter $j$, initially set to $1$, that indicates
    the index of the next bit that must be read in each $n_i$;

  \item $M$ stores the initial state $q_0$ of $A$;

  \item $M$ iteratively fetches bits $n_1(j), n_2(j), \ldots,
    n_d(j)$;\label{itm:tm:fetch}

  \item $M$ simulates one step of $A$ on $(n_1(j), n_2(j), \ldots,
    n_d(j))$, and updates the state of $A$;

  \item $M$ increments $j$ and repeats step~\ref{itm:tm:fetch} until
    all bits have been fetched;

  \item $M$ accepts its input iff the state reached in $A$ is final.
  \end{enumerate}

  It is readily seen that $M$ accepts $L_\varphi$. The only detail of
  concern is that the $\bin(n_i)$'s may have different lengths. This
  can be addressed by implicitly producing ``$0$'' as a padding bit
  whenever $j$ exceeds the length of $\bin(n_i)$, \ie whenever the
  reading head hits the next ``\#'' before seeing $j$ cells.

  It remains to argue that $M$ works in logarithmic space. Let $n$ be
  the length of the input. Note that $\varphi$ and $d$ are both fixed,
  and hence independent from $n$. Thus, tuples $(n_1(i), n_2(i),
  \ldots, a_d(i))$ and states of $A$ take constant space and can be
  stored in the control states of $M$. Moreover, counter $j$ does not
  exceed $n$, so its binary encoding can be stored on a work tape of
  length $O(\log n)$.
\end{proof}

By Proposition~\ref{prop:PA}, we immediately get:

\begin{theorem}\label{thm:pa:upper:bound}
  Let $\PP$ be an oblivious consensus protocol whose step relation is
  expressible in Presburger arithmetic. If $\PP$ computes a number
  predicate $\varphi$, then $\varphi \in \NSPACE(n)$.
\end{theorem}

It follows immediately from the definition that the step relation of
population protocols is expressible in Presburger arithmetic, and so,
by Theorem~\ref{thm:pa:upper:bound}, they can only compute number
predicates in $\NSPACE(n)$. However, their expressive power is far
below $\NSPACE(n)$. Indeed, it was shown in~\cite{AADFP04} that they
can only compute predicates in $\NL$, and we can now even go a bit
further. Since population protocols compute exactly the predicates
expressible in Presburger arithmetic~\cite{AAER07}, by
Proposition~\ref{prop:PA} we have:

\begin{corollary}
  Population protocols can only compute predicates in
  $\DSPACE(\log n)$.
\end{corollary}



==> sec-expressive-power-oblivious.tex <==
We introduce a generic computational model following the
computation-by-consensus paradigm introduced in~\cite{AADFP04,AAER07}
for population protocols. Its main feature is the
requirement that the future behavior of a protocol depends only on the
current \emph{number} of agents in each state, and not on their
identities. In particular, the protocol is oblivious of past states
and of the identities of the agents.

An \emph{oblivious consensus protocol with
leaders} is a tuple $\PP = (Q, \Step, \Sigma, L, I, O)$ where
$Q, \Sigma, L, I, O$ re defined as for population protocols, and 
$\Step \subseteq \pop{Q} \times \pop{Q}$ is the \emph{step
relation} between populations, satisfying $|C| = |C'|$ for every
$(C, C') \in \Step$. 

We show that under a very weak assumption on the step relation,
oblivious protocols can only compute predicates in
$\NL$. The assumption is that the step relation itself is
computable in $\NL$. Observe that the step relation of a
consensus protocol with $k$ states can be seen as a predicate
of arity $2 k$.

\begin{theorem}\label{thm:gen:upper:bound}
  Let $\PP = (Q, \Step, \Sigma, I, L, O)$ be an oblivious protocol
  computing a predicate $\varphi$. If $\Step \in \NL$,
  then $\varphi \in \NL$.
\end{theorem}

\begin{proof}
  Let $\ell$ be the arity of $\varphi$. We show that there is a
  nondeterministic Turing machine, running in $\bigO(n)$ space, that
  decides, on input $\vec{x} \in \Nat^\ell$, whether $\varphi(\vec{x})
  = 1$ holds.

  Let $d \defeq |I(\vec{x})|$. Let $G = (V,
  E)$ be the graph where $V$ is the set of all configurations of $\PP$
  of size $d$, and $(\c, \c') \in E$ if{}f $\c \trans{} \c'$. Every
  node of $V$ can be stored using at most $\ell \cdot \log d$ space
  and so, since $\ell$ is fixed, in space $\bigO(\log d)$. Observe
  that, since $\c \trans{*} \c'$ implies $|\c| = |\c'|$, $V$ contains
  all configurations reachable from $\c_0$.

  We claim that $\varphi(\vec{x}) = 1$ if{}f $G$ contains a
  configuration $\c$ satisfying the two following properties:
  \begin{enumerate}
  \item $\c_0 \trans{*} \c$;\label{prop:reach}

  \item every configuration reachable from $\c$, including $\c$
    itself, is a $1$-consensus.\label{prop:consensus}
  \end{enumerate}
  If $\varphi(\vec{x}) = 1$, then such a configuration $\c$ exists by
  definition. For the other direction, assume some configuration $\c$
  satisfies both properties. By assumption, there exists a fair
  execution starting at $\c_0$ that converges to $1$. Thus, since
  $\PP$ is well-specified, every fair execution starting at $\c_0$
  converges to $1$, and so $\varphi(\vec{x}) = 1$.

  By the claim, it suffices to exhibit a nondeterministic Turing
  machine $\TM_{\ref{prop:reach}\ref{prop:consensus}}(\c)$ that
  runs in $\bigO(\log |\c|)$ space and accepts a configuration $\c$
  if{}f $\c$ satisfies properties~\ref{prop:reach}
  and~\ref{prop:consensus}.

  We first observe that there is a nondeterministic Turing machine
  $\TM(\c)$ that runs in $\bigO(\log |\c|)$ space and accepts the
  configurations $\c$ satisfying the following property:
  \begin{quote}
    there exists a configuration $\c'$ such that $\c \trans{*} \c'$
    and $\c'$ is \emph{not} a $1$-consensus.
  \end{quote}
  The machine $\TM(\c)$ starts at $\c$, guesses a path of
  configurations step by step, and checks that the final configuration
  $\c'$ is not a $1$-consensus. While guessing the path, the machine
  only stores two configurations at any given time, and so, since
  every configuration reachable from $\c$ has the same size as $\c$,
  and since $\Step \in \NL$, the machine only uses $\bigO(\log
  |\c|)$ space. Checking whether $\c'$ is not a 1-consensus can be
  done in constant space.

  Now we use the fact that space complexity classes are closed under
  complement~\cite{Imm88}. Since $\NL = \coNL$, there
  exists a nondeterministic Turing machine $ \overline{\TM}(\c)$ that,
  given as input a configuration $\c$, decides in $\bigO(\log |\c|)$
  space whether every configuration reachable from $\c$ is a
  consensus.

  The machine $\TM_{\ref{prop:reach}\ref{prop:consensus}}(\c)$ first
  guesses a configuration $\c'$ reachable from $\c$, proceeding as in
  the description of $\TM(\c)$, and then simulates
  $\overline{\TM}(\c')$. Clearly, the machine runs in $\bigO(\log
  |\c|)$ space.
\end{proof}

The assumption that $\Step \in \NL$ is very weak. It follows immediately from the
definitions that both population protocols and broadcast protocols are oblivious. 
We now show that the protocols with absence detectors of \cite{MichailS15}. We recall the definition of an absence detector, using the terminology of this paper.

A protocol with absence detector is a tuple $\PP = (Q, R, D, \Sigma, L, I, O)$, where all components but $D$ are defined as for population protocols, and $D \subseteq Q \times 2^{|Q|} \times Q$ is the \emph{detection transition function}. We write $q, Q' \mapsto q'$ to denote $(q, Q',q') \in D$
The step relation of a protocol with absence detector is defined as follows. A pair $(C, C')$ belongs to $\Step$ if{}f 
\begin{itemize}
\item there exists $(p, q) \mapsto (p', q') \in R$ such that $C \geq \multiset{p, q}$ and $C' = C
 \mminus \multiset{p, q} \mplus \multiset{p', q'}$; or
\item there exists  $(q, Q',q') \in D$ such that $C(q) \geq 1$, $\supp{C}=Q'$, and 
$C' = C \mminus \multiset{q} \mplus \multiset{q'}$.
\end{itemize}

\begin{corollary}
Broadcast protocols and protocols with absence detectors can only compute predicates
in $\NL$.
\end{corollary}






==> sec-temporary.tex <==
\alert{Old stuff moved from the main text. This file will be removed! If you want to keep something, move it into sec-appendix.}

\begin{proposition}
  The unary predicate $\varphi$, such that $\varphi(x) = 1$ if{}f $x$ is a power of two is computable by a broadcast
  protocol.
\end{proposition}

\begin{IEEEproof}
  We define the protocol $\PP_\varphi = (Q, R, B, \Sigma, I, O)$
  computing $\varphi$ as follows: \michael{The protocol is not
    well-specified, if the input is a power of two, then it is
    possible to reach a configuration with a single $x$ and no $x'$;
    then one can move in one step to consensus $1$ or in two steps to
    consensus 0.}
  \newcommand{\remainder}{\mathtt{remainder}}
  \renewcommand{\error}{\mathtt{error}}
  \newcommand{\ToZero}{\textit{Move-to-zero}}
  \newcommand{\ToOne}{\textit{Move-to-one}}
  \newcommand{\ResetInit}{\textit{Reset}}
  \newcommand{\Halve}{\textit{Halve}}
  \newcommand{\zeroq}{\mathtt{zero}} \newcommand{\oneq}{\mathtt{one}}
  \begin{itemize}
  \item $Q \defeq \{x, x', \zeroq, \oneq, \error\}$;

  \item $R$ contains the transition $(x', x') \mapsto (x, \zero)$;

  \item $B$ contains four transitions,
  $$\begin{array}{lcl}
  x \mapsto x'; \Halve      & \quad & x' \mapsto \zeroq; \ToZero \\
  x \mapsto \oneq; \ToOne &          & \error \mapsto x; \ResetInit
  \end{array}$$
  \noindent where the transfer functions are defined as follows:
    \begin{align*}
      \Halve(q) &\defeq
      \begin{cases}
        x'     & \text{if}\ q = x, \\
        \error & \text{if}\ q = x',\\
        q & \text{ otherwise.}
      \end{cases} \\
      %
      \ToZero(q) &\defeq
      \begin{cases}
        \error & \text{if}\ q \in \{x', \error\}, \\
        \zeroq & \text{otherwise}.
      \end{cases} \\
      %
      \ToOne(q) &\defeq
      \begin{cases}
        \error & \text{if}\ q \in \{x, x', \error\}, \\
        \oneq  & \text{otherwise}.
      \end{cases} \\
      %
      \ResetInit(q) &= x\ \text{for every}\ q \in Q;
    \end{align*}

  \item $\Sigma \defeq \{x\}$;

  \item $I$ is the identity function;

  \item $O(q) \defeq
    \begin{cases}
      1 & \text{if}\ q = \oneq, \\
      0 & \text{otherwise}.
    \end{cases}$
  \end{itemize}

  The broadcast associated with $\Halve$ transfers agents from state
  $x$ to state $x'$, which starts the process of halving the
  number of agents in $x$ by means of the 
  single rendez-vous transition $(x', x')
  \mapsto (x, \zero)$. A reduction is finished if the rendez-vous
  transition is no longer enabled. Then, another reduction may be
  initiated by means of the broadcast associated with $\Halve$.  If
  the computation reaches a configuration $C$ such that $C(x') > 0$,
  then either a reduction is not finished at $C$, or the number of
  agents in $x$ was odd before the reduction started and $C(x') =
  1$. In either case, the initiation of another reduction is not
  permitted: Applying the broadcast associated with $\Halve$ at $C$
  transfers at least one agent into state $\error$; every agent in
  state $\error$ can reset the computation to the initial
  configuration by means of the broadcast associated with
  $\ResetInit$.

  An agent in state $x$ can non-determinisically guess that it is the
  \emph{only} agent remaining in state $x$, which implies that the
  initial number of agents in state $x$ was indeed a power of $2$, and
  convert everyone to state $\oneq$, by means of the broadcast
  associated with $\ToOne$. Analogously, an agent in state $x'$ can
  non-deterministically guess that it is the \emph{only} remaining
  agent in $x'$, which implies that the initial number of agents in
  state $x$ was not a power of $2$, and convert everyone to state
  $\zeroq$ by means of the broadcast associated with $\ToZero$.  If
  one of the two guesses is correct, the computation stabilizes to the
  correct output $O(\oneq) = 1$ or $O(\zeroq) = 0$, respectively.  If
  one of the two guesses is wrong, then at least one agent transitions
  to state $\error$ and by fairness will eventually reset the
  computation. Fairness ensures that the computation eventually
  stabilizes to the correct output.
\end{IEEEproof}

\subsubsection{Simulation of polynomially bounded counter machines by $n$-bounded counter machines}

\begin{lemma}
  For every polynomially bounded counter machine that computes some
  predicate $\varphi$, there exists an input-bound counter machine
  that computes $\varphi$.
\end{lemma}

Let $c$ be a positive constant and let $x$ be a counter such that
$C(x) \leq n^c$ for every configuration $C$ reachable from an input
configuration of input size $n$. Fix $C$.

We can express value of $x$ in base $n$ with $(c+1)$ coefficients:
$C(x) = \sum_{i=0}^{c+1}\alpha_i n^i$ with $0 \leq \alpha_i \leq (n-1)$.
We may rewrite this representation in matrix form to
$$
C(x) = \begin{bmatrix}
                 \mathbf{b_1} \\
                 \vdots \\
                 \mathbf{b_n}
                 \end{bmatrix} \cdot
                 \begin{bmatrix}
                   n^0 \\
                   \vdots \\
                   n^c
                 \end{bmatrix}
$$
with row vectors $\mathbf{b_i} \in \{0,1\}^{(c+1)}$ and $\sum_{i=1}^n b_{ji} = \alpha_j \leq (n-1)$ for
all $0 \leq j \leq (c+1)$.

Thus we may represent the value of a single $n^c$-bounded counter $x$
by means of multiple $n$-bounded counters $\{ x_\mathbf{b} \mid \mathbf{b} \in \{0,1\}^{(c+1)} \}$ where
the value of $x_\mathbf{b}$ is equal to the number of occurences of $\mathbf{b}$
among the row-vectors $\mathbf{b_1}, \ldots, \mathbf{b_n}$.
Notice that this representation is not unique, but this is of no concern for our
construction.

It remains to show how to implement the actions $\incr_x, \decr_x, \zero_x, \nonzero_x$
in this new presentation with these $2^{c+1}$ counters.
To simplify representation, we introduce sequential composition of transitions:
If $q, q'$ are states in some existing counting machine and $a_1$, \ldots, $a_n$ are
actions, then
$q \trans{a_1; a_2; \ldots; a_{m-1}; a_m} q'$ denotes the following operation:
Introduce new pairwise distinct states $q_1$ up to $q_{m-1}$ and add the transitions
$q_0 \trans{a_1} q_1, q_1 \trans{a_2} q_2, \ldots, q_{m-1} \trans{a_m} q_m$ with
$q_0 = q$ and $q_m = q'$. Let $x$ be a counter and let $0 < i \leq m$.
Add the following transitions, depending on $a_i$:
\begin{itemize}
  \item $a_i = \zero_x$: Add the transition $q_{i-1} \trans{\nonzero_x} q$.
  \item $a_i = \nonzero_x$: Add the transition $q_{i-1} \trans{\zero_x} q$.
  \item $a_i = \trans{\decr_x} q$: Add the transition $q_{i-1} \trans{\zero_x} q$.
\end{itemize}
This ensures that the execution of the composition does not get stuck in an auxiliary state if an
intermediate action cannot be executed.
For an ordered finite set $B = \{x_1, \ldots, x_n\}$ of counters, we write
$\trans{\zero(B)}$ as shorthand for $\trans{\zero(x_1); \ldots ;\zero(x_n)}$.
For $n < 2^{c+1}$, let $\mathtt{bin}(n) \in {0,1}^{(c+1)}$ denote the binary representation
of $n$ with least significant bit first.


\begin{itemize}
  \item $\nonzero_x $:
  $C(x) > 0$ iff. $\mathbf{b}_i \neq \mathbf{0}$ for at least
  one index $1 \leq i \leq n$. Thus the nonzero test in the new implemention
  has to check if the counter value of $x_\mathbf{b}$
  is positive for at least one $\mathbf{b} \neq \mathbf{0}$:
  We replace every transition $q \trans{\nonzero_x} z$
  in the former protocol by
  $$\bigcup_{\mathbf{b} \in \{0,1\}^c, \mathbf{b} \neq \mathbf{0}} (q, \nonzero_{x_b}, z)$$.
  \item $\zero_x $:
        Let $q \trans{\zero_x} z$ be a transition in the original protocol.
        $C(x) = 0$ iff.
        $\mathbf{b}_i = \mathbf{0}$ for all $1 \leq i \leq n$.
        Thus for every $\mathbf{b} \in \{0,1\}^{(C+1)} \setminus \{\mathbf{0}\}$ we have to
        check if the value of $x_{\mathbf{b}}$ equals $0$. This can be implemented by means of the composition
       $q \trans{\zero_{x_{\bin(1)}};\zero_{x_{\bin(2)}}; \ldots; \zero_{x_{\bin(2^{c+1}-1)}}} z$.
  \item $\incr_x$: Incrementing $C(x)=\sum_{i=0}^{c+1}\alpha_i n^i$
        by one boils down to incrementing $\alpha_0$ by one.
        This, in turn, boils down to flipping one left-most bit from exactly one of the vectors
        $\mathbf{b}_i$ from $0$ to $1$. If no such vector with the left-most bit equalling $0$
        exists, this means $\alpha_0 = n-1$,
        and an overflow occurs. An overflow is handled by setting the left-most bit of \emph{all}
        row vectors $\mathbf{b}_i$ to $0$ and
        then flipping the second bit of exactly one of the resulting vectors from
        $0$ to $1$. Of course, it could be the case that again an overflow occurs.
        Such an overflow is
        handled in an analogous manner (setting the second bit of all vectors to $0$ and
        flipping the third bit of precisely one vector from $0$ to $1$).
        This way we cascade the carry to the third bit, and so forth,
        until no more overflow occurs.
        Since $x$ is $n^c$-bounded, we are guaranteed that no overflow occurs when we try to flip
        the right-most bit from $0$ to $1$.

        Let $(q, \incr_x, r)$ be a transition in the original protocol.
        We introduce auxiliary states
        $$\{(q, \incr \, i, x_b), (q, \mathtt{unset } \, i, x_b),
        \mid i \in \{ 1, \ldots, c+1\}, b \in \{0,1\}^c \}$$
        Intuitively, if the machine is in a state of the form
         $(q, \incr \, i, x_b)$,
        then it attempts to increment the $i$th bit of precisely one of the duplicates of the
        row vector $\mathbf{b}$. If the machine is in a state of the form
        $(q, \mathtt{unset} \, i, x_b)$, then it attempts to unset the $i$th bit of \emph{all}
        duplicates of the vector $\mathbf{b}$ to zero.

        More precisely, if the machine is in state $(q, \incr \, i, x_b)$,
        it performs the following steps in succession:
        \begin{enumerate}
          \item If $\mathbf{b}=1^n$: This indicates that an overflow occured, so transition to state $(q, \mathtt{unset \, i, x_\mathbf{0}})$.
                \label{step_zero}
          \item If the $i$th left-most bit of the vector $\mathbf{b}$ is equal to $1$
                or the value of $x_b$ is equal to $0$:
                Transition to state $(q, \incr \, i, x_{(b \oplus 1)})$.
                \label{step_one}
          \item  Otherwise:
                 \begin{enumerate}
                   \item Decrement the value of $x_b$ by one.
                         \label{step_two}
                   \item Increment the value of $x_{b+\mathbf{e_i}}$ by one
                         and transition to the original target state $z$.
                         \label{step_three}
                 \end{enumerate}
        \end{enumerate}

        This sequence of steps is realized by adding the following transitions:
        \begin{align}
        & (q, \incr \, i, x_{\mathbf{1}}) \trans{\nop} (q, \mathtt{unset} \, i, x_{\mathbf{0}}) & \label{trans_zero} \\
        & (q, \incr \, i, x_b) \trans{\zero_{x_b}} (q, \incr \, i, x_{b \oplus 1}) & \text{ for all } \mathbf{b}\neq \mathbf{1} \text{ and } i, \label{trans_one}\\
        & (q, \incr \, i, x_b) \trans{\nop} (q, \incr \, i, x_{b \oplus 1}) & \text{ for all } \mathbf{b} \neq \mathbf{1} \text{ s.t. } b_i \neq 0, \label{trans_two}\\
        & (q, \incr \, i, x_b) \trans{\decr_{x_\mathbf{b}}; \incr_{x_{(\mathbf{b}+\mathbf{e}_i)}}} z & \text{ for all } \mathbf{b}\neq \mathbf{1} \text{ s.t. } b_i = 0, \label{trans_three}
        \end{align}

        where (\ref{trans_zero}) implements Step \ref{step_zero}, (\ref{trans_one})
        and (\ref{trans_two}) implement Step \ref{step_one},
        and (\ref{trans_three}) implements steps \ref{step_two} and \ref{step_three}.

        If the machine is in state $(q, \mathtt{unset} \, i, x_b)$, it performs the following
        sequence of steps to unset the $i$th bit of all duplicates of $\mathbf{b}$:

        \begin{enumerate}
          \item If $\mathbf{b} = 1^{(c+1)}$, then transition to state $(q, \incr \, (i+1), x_{\mathbf{0}})$. \label{unset_step_zero}
          \item If the value of $x_{\mathbf{b}}$ equals $0$ or the $i$th bit of $\mathbf{b}$ equals
                $0$, transition to state $(q, \mathtt{unset} \, (i+1), x_{(\mathbf{b} \oplus 1)})$. \label{unset_step_one}
          \item Otherwise:
                \begin{enumerate}
                  \item Decrement $x_{\mathbf{b}}$ by one. \label{unset_step_two}
                  \item Increment $x_{\mathbf{b} - \mathbf{e}_i}$ by one and transition back to
                        state $(q, \mathtt{unset} \, i, x_b)$. \label{unset_step_three}
                \end{enumerate}
        \end{enumerate}

        This sequence of steps is realized by adding the following transitions:

        \begin{align}
        & (q, \mathtt{unset} \, i, x_{\mathbf{1}}) \trans{\nop} (q, \incr \, (i+1), x_{\mathbf{0}}) & \text{ for all } i < c, \label{t_unset_0}\\
        & (q, \mathtt{unset} \, i, x_\mathbf{b}) \trans{\zero_{x_\mathbf{b}}}  (q, \mathtt{unset} \, i, x_{(\mathbf{b} \oplus 1)}) & \text{ for all } \mathbf{b} \neq \mathbf{1} \text{ and }  i < c, \label{t_unset_1} \\
        & (q, \mathtt{unset} \, i, x_\mathbf{b}) \trans{\nop}  (q, \mathtt{unset} \, i, x_{(\mathbf{b} \oplus 1)} & \text{ for all } \mathbf{b} \text{ s.t. } b_i = 0 \label{t_unset_2}\\
        & (q, \mathtt{unset} \, i, x_\mathbf{b}) \trans{\decr_{x_\mathbf{b}}; \incr_{x_{\mathbf{b}-\mathbf{e}_i}}} (q, \mathtt{unset} \, i, x_b)  & \text{ for all } \mathbf{b} \text{ s.t. } b_i = 1. \label{t_unset_3}
      \end{align}

      where (\ref{t_unset_0}) implements Step \ref{unset_step_zero}, (\ref{t_unset_1})
      implements Step \ref{unset_step_one},  (\ref{t_unset_2}) implements \ref{unset_step_two},
      and (\ref{t_unset_3}) implements Step \ref{unset_step_three}.

      Finally, we replace the original transition $q \trans{\incr_x} z$ by $q \trans{\nop} (q, \incr \, 1, x_\mathbf{0})$.
  \item $\mathbf{decr}_x$
     Decrementing the value of $x$ in our new representation boils down to the following sequence of steps:
     \begin{enumerate}
       \item Find the smallest index $i$, $1 \leq i \leq c$, such that there exists
            some $\mathbf{b} \in \{0, 1\}^{(c+1)}$ where the value of
             $x_{\mathbf{b}}$ is positive and $b_{i} > 0$. If there is no such index $i$, abort.
             \label{decr_step_0}
       \item Decrement value of $x_{\mathbf{b}}$ for some $\mathbf{b}$ where $b_i = 1$.
             \label{decr_step_1}
       \item If $i > 1$, set the $(i-1)$th bit of all vectors to $1$, i.e.
             add counter value of $x_\mathbf{b}$ to the value of $x_\mathbf{b+\mathbf{e}_{(i-1)}}$
             and set counter value of  $x_\mathbf{b}$ to zero for all $\mathbf{b}$
             where $b_{i-1} = 0$.
             \label{decr_step_2}
     \end{enumerate}


     For $\mathbf{b} = b_1 \ldots b_{c+1} \in \{0,1\}^{(c+1)} \setminus 0^*$, let
     $r(\mathbf{b})$ denote the smallest index $i$ such that $b_i = 1$ and
     let $R_i \defeq \{\mathbf{b}  \in \{0,1\}^{(c+1)} \mid r(\mathbf{b}) = i \}$.


     The sequence of steps is realized by adding the following sequence of
     transitions:
     \begin{align}
       & q \trans{\zero_{x_{\mathtt{bin}(1)}}; \ldots; \zero_{x_{\mathtt{bin}(n-1)}}; \nonzero_{x_{\mathtt{bin}(n)}}} q_n \text{ for all } 0 < n < 2^{(c+1)} \label{decr_trans_0}\\
       & q_n \trans{\decr_{x_{\mathtt{bin}(n)}}} z_i \text { for all } 0 < n < 2^{(c+1)} \text{ s.t. } r\left(\mathtt{bin}(n)\right) = i\label{decr_trans_1} \\
       & z_i \trans{\decr_{x_\mathbf{b}}; \incr_{x_{\mathbf{b} \oplus \mathbf{e}_{i-1} }}} z_i \text{ for all } 1 < i \leq  c,  \mathbf{b} \in R_{i+1}\label{decr_trans_2} \\
       & z_i \trans{\zero(R_{i+1})} z \text{ for all } 0 < i < c\label{decr_trans_3}
    \end{align}
    where $q_i$ and $z_i$ are additional helper states for every $0 < i < c$;
    transition (\ref{decr_trans_0}) implements Step \ref{decr_step_0}, (\ref{decr_trans_1})
    implements step \ref{decr_step_2}, and transitions (\ref{decr_trans_2}) and
    (\ref{decr_trans_3}) implement Step \ref{decr_step_2}.
\end{itemize}

